Cyberphysical Blockchain-Enabled Peer-to-Peer Energy Trading

Scalability and security problems of the centralized architecture models in cyberphysical systems have great potential to be solved by novel blockchain based distributed models.A decentralized energy trading system takes advantage of various sources and effectively coordinates the energy to ensure optimal utilization of the available resources. It achieves that goal by managing physical, social and business infrastructures using technologies such as Internet of Things (IoT), cloud computing and network systems. Addressing the importance of blockchain-enabled energy trading in the context of cyberphysical systems, this article provides a thorough overview of the P2P energy trading and the utilization of blockchain to enhance the efficiency and the overall performance including the degree of decentralization, scalability and the security of the systems. Three blockchain based energy trading models have been proposed to overcome the technical challenges and market barriers for better adoption of this disruptive technology.

==> Sections/old-3_relatedwork.tex <==
\section{Related Work}

% Due to the fast innovation in the field of Blockchain, it has found its way in many energy trading applications. Blockchain has revolutionized the concept of security, transparency and sustainability in the energy sector. There are number of applications including, grid management, security and the accountability of the grads, efficient utility billing process and P2P energy trading. There are number of papers and articles that discuss the different methods and the infrastructures for efficient use of blockchain. Several papers discuss various aspects of peer-to-peer distributed energy trading. Mostly, they discuss the challenges in the energy sharing paradigm and the architectures that give the solutions for energy management, improving the trading trust and regularized billing schemes. These papers do not discuss the blockchain based energy trading solutoins. To summarize the concepts use in the blockchain papers, articles and the businesses, number of surveys and review papers have been presented. [CITE THE PAPERS]. 

\begin{figure}[]
\centerline{\includegraphics[width=\columnwidth]{./Pictures/wang2019energy.PNG}}
\caption{Blockchain based energy trading.}
\label{fig1}
\end{figure}

 The papers also talks about he existing energy schemes and discuss the case studies as well. In addition, paper gives a Blockchain-Based Smart Contract System for Energy Saving Certificates. \cite{abdella2018peer} discuss a little about the advantages of introducing the blockchain in the systems but the main purpose of the review is to present the existing P2P research which does not involve blockchain. The topics covered include architecture of P2P DET, demand response optimization models, power routing devices and algorithms. \cite{chitchyan2018review} describe the current trends of blockchain in the energy sharing. The paper does not compare and discuss the challenges in adoption of blockchain and future research.

% \cite{o2019systematic} gives a analytical rather than technical overview of the blockchain solutions. The research objectives of paper are determining growth
% rates, failure rates
% and trends in the businesses, determining method of
% sharing information, determining depth of
% technical information and determining technical
% trends (meaning which blockchain platform is used, which consensus being used etc). The paper category the blockchain projects in different fields including the country, year and the research problem of the project. Then paper determines the trends listed above in these projects. 


% In this regard, \cite{wang2019energy, andoni2019blockchain} give very in depth and detailed review of the DLT in energy sector. \cite{andoni2019blockchain} discusses 140 research and industrial papers and initiatives. They presented an overview on the
% fundamentals of blockchain technologies, including system architectures and distributed consensus algorithms, critical components of
% performance for blockchain ecosystems. They also presented and compared the usecases of blockchain and showcased the trends of stakeholders and industrial businesses in the development of blockhiain solutions. Whereas \cite{wang2019energy} divides the the energy trading paradigm in the sub-classes shown in fig \ref{fig1} and then discusses the contributions in each subclass. The paper presents the solutions to improves the parts of the architecture rather than the complete projects that are  already deployed.

% Most of these review papers discuss the overall impact of the blockchain in the energy industry. Our paper will be focusing on the fined grained analysis of the solutions and the architectures related to the P2P distributed energy trading involving blockchain.  \cite{zhang2017review} is based on the discussion of 10 blockchain initiatives and compare those projects. Although, this paper does not discuss in depth about the technological advancements and challenges for the blockchain based P2P energy trading proposals. \cite{sousa2019peer} talks about potential of P2P energy sharing and the businesses which are dealing with distributed energy. Paper divides the projects in three categories, full P2P energy trading, community-based market and hybrid model. The paper does not talk about the blockchain applications. 


